pDANSE: Particle-based Data-driven Nonlinear State Estimation from Nonlinear Measurements

We consider the problem of designing a data-driven nonlinear state estimation (DANSE) method that uses (noisy) nonlinear measurements of a process whose underlying state transition model (STM) is unknown. Such a process is referred to as a model-free process. A recurrent neural network (RNN) provides parameters of a Gaussian prior that characterize the state of the model-free process, using all previous measurements at a given time point. In the case of DANSE, the measurement system was linear, leading to a closed-form solution for the state posterior. However, the presence of a nonlinear measurement system renders a closed-form solution infeasible. Instead, the secondorder statistics of the state posterior are computed using the nonlinear measurements observed at the time point. We address the nonlinear measurements using a reparameterization trickbased particle sampling approach, and estimate the second-order statistics of the state posterior. The proposed method is referred to as particle-based DANSE (pDANSE). The RNN of pDANSE uses sequential measurements efficiently and avoids the use of computationally intensive sequential Monte-Carlo (SMC) and/or ancestral sampling. We describe the semi-supervised learning method for pDANSE, which transitions to unsupervised learning in the absence of labeled data. Using a stochastic Lorenz-63 system as a benchmark process, we experimentally demonstrate the state estimation performance for four nonlinear measurement systems. We explore cubic nonlinearity and a cameramodel nonlinearity where unsupervised learning is used; then we explore half-wave rectification nonlinearity and Cartesian-tospherical nonlinearity where semi-supervised learning is used. Additionally, we also show the performance of pDANSE for the stochastic Lorenz-96 system with a half-wave, rectified measurement system. The performance of state estimation is shown to be competitive vis-a-vis model-driven methods that have complete knowledge of the STM of the dynamical system.

==> figs/NMSE_vs_Lorenz63.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{green01270}{RGB}{0,127,0}
\definecolor{lightgray204}{RGB}{204,204,204}

\begin{axis}[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.5,0.09)},
  anchor=south,
  draw=lightgray204
},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={SMNR (in dB)},
xmajorgrids,
xmin=-1.5, xmax=31.5,
xtick style={color=black},
y grid style={darkgray176},
ylabel={NMSE (in dB)},
ymajorgrids,
ymin=-33.5597082292661, ymax=-3.4059056667611,
ytick style={color=black}
]
\begin{comment}
\path [draw=green01270, semithick]
(axis cs:0,4.1323341652751)
--(axis cs:0,4.38153988867998);

\path [draw=green01270, semithick]
(axis cs:10,0.238507971167564)
--(axis cs:10,0.553816094994545);

\path [draw=green01270, semithick]
(axis cs:20,-2.46001968532801)
--(axis cs:20,-2.29030837863684);

\path [draw=green01270, semithick]
(axis cs:30,9.26267306879163)
--(axis cs:30,9.36201412603259);
\end{comment}
\path [draw=red, semithick]
(axis cs:0,-8.60902464389801)
--(axis cs:0,-6.28654420375824);

\path [draw=red, semithick]
(axis cs:10,-15.2147521972656)
--(axis cs:10,-9.18701934814453);

\path [draw=red, semithick]
(axis cs:20,-26.2827706336975)
--(axis cs:20,-13.2057089805603);

\path [draw=red, semithick]
(axis cs:30,-31.5158166885376)
--(axis cs:30,-16.4359922409058);

\path [draw=black, semithick]
(axis cs:0,-5.50212812423706)
--(axis cs:0,-5.05350542068481);

\path [draw=black, semithick]
(axis cs:10,-10.128625869751)
--(axis cs:10,-7.9116153717041);

\path [draw=black, semithick]
(axis cs:20,-17.2814559936523)
--(axis cs:20,-9.91721343994141);

\path [draw=black, semithick]
(axis cs:30,-26.7276694774628)
--(axis cs:30,-23.7606880664825);

\path [draw=blue, semithick]
(axis cs:0,-5.48225319385529)
--(axis cs:0,-4.51392447948456);

\path [draw=blue, semithick]
(axis cs:10,-14.784937620163)
--(axis cs:10,-10.6168549060822);

\path [draw=blue, semithick]
(axis cs:20,-21.6732284724712)
--(axis cs:20,-21.1052520573139);

\path [draw=blue, semithick]
(axis cs:30,-24.3280916213989)
--(axis cs:30,-23.2241201400757);

%\addplot [semithick, green01270, dash pattern=on 1pt off 3pt on 3pt off 3pt, mark=pentagon*, mark size=3, mark options={solid}]
%table {%
%0 4.25693702697754
%10 0.396162033081055
%20 -2.37516403198242
%30 9.31234359741211
%};
%\addlegendentry{DANSE_SEMISUPERVISED_PLUS}
\addplot [semithick, red, dashed, mark=diamond*, mark size=3, mark options={solid}]
table {%
0 -7.44778442382812
10 -12.2008857727051
20 -19.7442398071289
30 -23.9759044647217
};
\addlegendentry{PF}
\addplot [semithick, black, dashed, mark=square*, mark size=3, mark options={solid}]
table {%
0 -5.27781677246094
10 -9.02012062072754
20 -13.5993347167969
30 -25.2441787719727
};
\addlegendentry{DANSE (Sup.) $\kappa=2\%$}
\addplot [semithick, blue, mark=*, mark size=3, mark options={solid}]
table {%
0 -4.99808883666992
10 -12.7008962631226
20 -21.3892402648926
30 -23.7761058807373
};
\addlegendentry{$\text{SemiDANSE}+$ $\kappa=2\%$}
\end{axis}

\end{tikzpicture}


==> figs/journalpaper/cart2sph3d/nmse_pf_pdanse_nsup_all_cart2sph3dmod.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkviolet1910191}{RGB}{191,0,191}
\definecolor{lightgray204}{RGB}{204,204,204}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={SMNR (in dB)},
xmajorgrids,
xmin=-1.5, xmax=31.5,
xtick style={color=black},
xtick={-5,0,5,10,15,20,25,30,35},
xticklabels={
  \(\displaystyle {\ensuremath{-}5}\),
  \(\displaystyle {0}\),
  \(\displaystyle {5}\),
  \(\displaystyle {10}\),
  \(\displaystyle {15}\),
  \(\displaystyle {20}\),
  \(\displaystyle {25}\),
  \(\displaystyle {30}\),
  \(\displaystyle {35}\)
},
y grid style={darkgray176},
ylabel={NMSE (in dB)},
ymajorgrids,
ymin=-31.8889794200659, ymax=-0.632319286465645,
ytick style={color=black},
ytick={-35,-30,-25,-20,-15,-10,-5,0},
yticklabels={
  \(\displaystyle {\ensuremath{-}35}\),
  \(\displaystyle {\ensuremath{-}30}\),
  \(\displaystyle {\ensuremath{-}25}\),
  \(\displaystyle {\ensuremath{-}20}\),
  \(\displaystyle {\ensuremath{-}15}\),
  \(\displaystyle {\ensuremath{-}10}\),
  \(\displaystyle {\ensuremath{-}5}\),
  \(\displaystyle {0}\)
},
width=\linewidth,
height=0.75\linewidth
]
\path [draw=red, semithick]
(axis cs:0,-8.45058465003967)
--(axis cs:0,-6.33879446983337);

\path [draw=red, semithick]
(axis cs:10,-16.7247097492218)
--(axis cs:10,-9.80679774284363);

\path [draw=red, semithick]
(axis cs:20,-24.860981464386)
--(axis cs:20,-12.3047366142273);

\path [draw=red, semithick]
(axis cs:30,-30.4682221412659)
--(axis cs:30,-16.9258208274841);

\path [draw=blue, semithick]
(axis cs:0,-2.72164267301559)
--(axis cs:0,-2.05307656526566);

\path [draw=blue, semithick]
(axis cs:10,-13.0960295200348)
--(axis cs:10,-10.5998494625092);

\path [draw=blue, semithick]
(axis cs:20,-20.6505264937878)
--(axis cs:20,-20.1248336136341);

\path [draw=blue, semithick]
(axis cs:30,-23.3176446706057)
--(axis cs:30,-22.8266538828611);

\path [draw=darkviolet1910191, semithick]
(axis cs:0,-5.08486556261778)
--(axis cs:0,-4.84069062024355);

\path [draw=darkviolet1910191, semithick]
(axis cs:10,-12.8024277091026)
--(axis cs:10,-11.2014556527138);

\path [draw=darkviolet1910191, semithick]
(axis cs:20,-17.650169044733)
--(axis cs:20,-17.180153220892);

\path [draw=darkviolet1910191, semithick]
(axis cs:30,-19.2828558087349)
--(axis cs:30,-18.6476327776909);

\addplot [thick, red, mark=diamond, mark size=5, mark options={solid,fill opacity=0}]
table {%
0 -7.39468955993652
10 -13.2657537460327
20 -18.5828590393066
30 -23.697021484375
};
\addlegendentry{$\textrm{PF}$}
\addplot [thick, blue, mark=o, mark size=4, mark options={solid,fill opacity=0}]
table {%
0 -2.38735961914062
10 -11.847939491272
20 -20.3876800537109
30 -23.0721492767334
};
\addlegendentry{$\textrm{pDANSE}$ $(\kappa=0\%)$}
\addplot [thick, darkviolet1910191, mark=square, mark size=4, mark options={solid,fill opacity=0}]
table {%
0 -4.96277809143066
10 -12.0019416809082
20 -17.4151611328125
30 -18.9652442932129
};
\addlegendentry{$\textrm{pDANSE}$ $(\kappa=2\%)$}
\end{axis}

\end{tikzpicture}


==> figs/journalpaper/cart2sph3d/revision_1/pdanse_supervised/nmse_pf_pdanse_nsup_20_w_supervised_all_cart2sph3dmod.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{lightgray204}{RGB}{204,204,204}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={SMNR (in dB)},
xmajorgrids,
xmin=-1.5, xmax=31.5,
xtick style={color=black},
xtick={-5,0,5,10,15,20,25,30,35},
xticklabels={
  \(\displaystyle {\ensuremath{-}5}\),
  \(\displaystyle {0}\),
  \(\displaystyle {5}\),
  \(\displaystyle {10}\),
  \(\displaystyle {15}\),
  \(\displaystyle {20}\),
  \(\displaystyle {25}\),
  \(\displaystyle {30}\),
  \(\displaystyle {35}\)
},
y grid style={darkgray176},
ylabel={NMSE (in dB)},
ymajorgrids,
ymin=-31.7496179271489, ymax=-3.55891063772142,
ytick style={color=black},
ytick={-35,-30,-25,-20,-15,-10,-5,0},
yticklabels={
  \(\displaystyle {\ensuremath{-}35}\),
  \(\displaystyle {\ensuremath{-}30}\),
  \(\displaystyle {\ensuremath{-}25}\),
  \(\displaystyle {\ensuremath{-}20}\),
  \(\displaystyle {\ensuremath{-}15}\),
  \(\displaystyle {\ensuremath{-}10}\),
  \(\displaystyle {\ensuremath{-}5}\),
  \(\displaystyle {0}\)
}
]
\path [draw=red, semithick]
(axis cs:0,-8.45058465003967)
--(axis cs:0,-6.33879446983337);

\path [draw=red, semithick]
(axis cs:10,-16.7247097492218)
--(axis cs:10,-9.80679774284363);

\path [draw=red, semithick]
(axis cs:20,-24.860981464386)
--(axis cs:20,-12.3047366142273);

\path [draw=red, semithick]
(axis cs:30,-30.4682221412659)
--(axis cs:30,-16.9258208274841);

\path [draw=blue, semithick]
(axis cs:0,-5.08457455784082)
--(axis cs:0,-4.84030642360449);

\path [draw=blue, semithick]
(axis cs:10,-12.8023664951324)
--(axis cs:10,-11.2013185024261);

\path [draw=blue, semithick]
(axis cs:20,-17.4711494594812)
--(axis cs:20,-16.9983177036047);

\path [draw=blue, semithick]
(axis cs:30,-19.022018879652)
--(axis cs:30,-18.3873515427113);

\path [draw=blue, semithick]
(axis cs:0,-5.66081640124321)
--(axis cs:0,-5.30013254284859);

\path [draw=blue, semithick]
(axis cs:10,-8.40075504779816)
--(axis cs:10,-5.81379497051239);

\path [draw=blue, semithick]
(axis cs:20,-15.9777939319611)
--(axis cs:20,-10.9312388896942);

\path [draw=blue, semithick]
(axis cs:30,-22.6628280878067)
--(axis cs:30,-19.1378272771835);

\addplot [semithick, red, mark=diamond, mark size=5, mark options={solid,fill opacity=0}]
table {%
0 -7.39468955993652
10 -13.2657537460327
20 -18.5828590393066
30 -23.697021484375
};
\addlegendentry{$\textrm{pDANSE-Sup.}$ $(\kappa=2.0\%)$}
\addplot [semithick, blue, mark=o, mark size=6, mark options={solid,fill opacity=0}]
table {%
0 -4.96244049072266
10 -12.0018424987793
20 -17.234733581543
30 -18.7046852111816
};
\addlegendentry{$\textrm{pDANSE-Sup.}$ $(\kappa=2.0\%)$}
\addplot [semithick, blue, dashed, mark=o, mark size=6, mark options={solid,fill opacity=0}]
table {%
0 -5.4804744720459
10 -7.10727500915527
20 -13.4545164108276
30 -20.9003276824951
};
\addlegendentry{$\textrm{pDANSE-Sup.}$ $(\kappa=2.0\%)$}
\end{axis}

\end{tikzpicture}


==> figs/journalpaper/cubic/nmse_pf_pdanse_nsup0_cubic.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{green01270}{RGB}{0,127,0}
\definecolor{lightgray204}{RGB}{204,204,204}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={SMNR (in dB)},
xmajorgrids,
xmin=-1.5, xmax=31.5,
xtick style={color=black},
xtick={-5,0,5,10,15,20,25,30,35},
xticklabels={
  \(\displaystyle {\ensuremath{-}5}\),
  \(\displaystyle {0}\),
  \(\displaystyle {5}\),
  \(\displaystyle {10}\),
  \(\displaystyle {15}\),
  \(\displaystyle {20}\),
  \(\displaystyle {25}\),
  \(\displaystyle {30}\),
  \(\displaystyle {35}\)
},
y grid style={darkgray176},
ylabel={NMSE (in dB)},
ymajorgrids,
ymin=-25.0539624214172, ymax=-3.80867033004761,
ytick style={color=black},
ytick={-27.5,-25,-22.5,-20,-17.5,-15,-12.5,-10,-7.5,-5,-2.5},
yticklabels={
  \(\displaystyle {\ensuremath{-}27.5}\),
  \(\displaystyle {\ensuremath{-}25.0}\),
  \(\displaystyle {\ensuremath{-}22.5}\),
  \(\displaystyle {\ensuremath{-}20.0}\),
  \(\displaystyle {\ensuremath{-}17.5}\),
  \(\displaystyle {\ensuremath{-}15.0}\),
  \(\displaystyle {\ensuremath{-}12.5}\),
  \(\displaystyle {\ensuremath{-}10.0}\),
  \(\displaystyle {\ensuremath{-}7.5}\),
  \(\displaystyle {\ensuremath{-}5.0}\),
  \(\displaystyle {\ensuremath{-}2.5}\)
},
width=\linewidth,
height=0.75\linewidth
]
\path [draw=red, thick]
(axis cs:0,-10.4346261024475)
--(axis cs:0,-7.12994337081909);

\path [draw=red, thick]
(axis cs:10,-15.8362140655518)
--(axis cs:10,-9.69286727905273);

\path [draw=red, thick]
(axis cs:20,-18.7608802318573)
--(axis cs:20,-10.8167831897736);

\path [draw=red, thick]
(axis cs:30,-21.2569842338562)
--(axis cs:30,-10.7379517555237);

\begin{comment}
\path [draw=green01270, thick]
(axis cs:0,-7.56243801116943)
--(axis cs:0,-4.77436542510986);

\path [draw=green01270, thick]
(axis cs:10,-11.9211685657501)
--(axis cs:10,-6.37612986564636);

\path [draw=green01270, thick]
(axis cs:20,-19.9295167922974)
--(axis cs:20,-11.1617727279663);

\path [draw=green01270, thick]
(axis cs:30,-24.088267326355)
--(axis cs:30,-18.5255098342896);
\end{comment}

\path [draw=blue, thick]
(axis cs:0,-5.68764507770538)
--(axis cs:0,-5.19779193401337);

\path [draw=blue, thick]
(axis cs:10,-8.446009516716)
--(axis cs:10,-7.47339737415314);

\path [draw=blue, thick]
(axis cs:20,-16.1877462863922)
--(axis cs:20,-14.7637422084808);

\path [draw=blue, thick]
(axis cs:30,-20.7465742230415)
--(axis cs:30,-19.2584039568901);

\addplot [thick, red, mark=diamond, mark size=4, mark options={solid,fill opacity=0}]
table {%
0 -8.7822847366333
10 -12.7645406723022
20 -14.7888317108154
30 -15.9974679946899
};
\addlegendentry{$\text{PF}$}
\begin{comment}
\addplot [thick, green01270, mark=square, mark size=4, mark options={solid,fill opacity=0}]
table {%
0 -6.16840171813965
10 -9.14864921569824
20 -15.5456447601318
30 -21.3068885803223
};
\addlegendentry{$\text{UKF}$}
\end{comment}
\addplot [thick, blue, mark=o, mark size=4, mark options={solid,fill opacity=0}]
table {%
0 -5.44271850585938
10 -7.95970344543457
20 -15.4757442474365
30 -20.0024890899658
};
\addlegendentry{$\text{pDANSE } (\kappa=0\%)$}
\end{axis}

\end{tikzpicture}


==> figs/journalpaper/highdim/nmse_vs_smnr_pdanse_nsup0.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{lightgray204}{RGB}{204,204,204}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={SMNR (in dB)},
xmajorgrids,
xmin=-0.5, xmax=10.5,
xtick style={color=black},
y grid style={darkgray176},
ylabel={NMSE (in dB)},
ymajorgrids,
ymin=-19.1250659331679, ymax=-10.7499110892415,
ytick style={color=black}
]
\path [draw=blue, semithick]
(axis cs:0,-11.811374694109)
--(axis cs:0,-11.1305999457836);

\path [draw=blue, semithick]
(axis cs:5,-15.7506991624832)
--(axis cs:5,-15.044096827507);

\path [draw=blue, semithick]
(axis cs:10,-18.7443770766258)
--(axis cs:10,-17.8340149521828);

\addplot [semithick, blue, mark=o, mark size=6, mark options={solid,fill opacity=0}]
table {%
0 -11.4709873199463
5 -15.3973979949951
10 -18.2891960144043
};
\addlegendentry{$pDANSE  (\kappa=0.0\%)$}
\end{axis}

\end{tikzpicture}


==> figs/nmse_pf_ukf_sdfail_sdk2.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{goldenrod1911910}{RGB}{191,191,0}
\definecolor{green01270}{RGB}{0,127,0}
\definecolor{lightgray204}{RGB}{204,204,204}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=0.75, text opacity=1, draw=lightgray204},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmajorgrids,
xmin=-1.5, xmax=31.5,
xtick style={color=black},
y grid style={darkgray176},
ymajorgrids,
ymin=-31.5343591690063, ymax=-1.20144395828247,
ytick style={color=black},
width=0.5\textwidth,
height=0.35\textwidth,
ylabel={NMSE (in dB)},
xlabel={SMNR (in dB)}
]
\begin{comment}
\path [draw=goldenrod1911910, semithick]
(axis cs:0,-12.4451358318329)
--(axis cs:0,-9.73202633857727);

\path [draw=goldenrod1911910, semithick]
(axis cs:10,-20.6974847316742)
--(axis cs:10,-14.4316046237946);

\path [draw=goldenrod1911910, semithick]
(axis cs:20,-26.7477426528931)
--(axis cs:20,-22.119101524353);

\path [draw=goldenrod1911910, semithick]
(axis cs:30,-30.1555902957916)
--(axis cs:30,-25.3924558162689);
\end{comment}
\path [draw=red, semithick]
(axis cs:0,-13.1015230417252)
--(axis cs:0,-10.1534723043442);

\path [draw=red, semithick]
(axis cs:10,-18.6489214897156)
--(axis cs:10,-12.0798077583313);

\path [draw=red, semithick]
(axis cs:20,-26.4155530929565)
--(axis cs:20,-15.9392290115356);

\path [draw=red, semithick]
(axis cs:30,-29.5748081207275)
--(axis cs:30,-17.8845081329346);

\path [draw=green01270, semithick]
(axis cs:0,-6.84911227226257)
--(axis cs:0,-2.58021283149719);

\path [draw=green01270, semithick]
(axis cs:10,-15.4501211643219)
--(axis cs:10,-14.4950692653656);

\path [draw=green01270, semithick]
(axis cs:20,-16.8100884258747)
--(axis cs:20,-16.0592887103558);

\path [draw=green01270, semithick]
(axis cs:30,-15.9933540821075)
--(axis cs:30,-15.3148143291473);

\path [draw=blue, semithick]
(axis cs:0,-11.8556115627289)
--(axis cs:0,-10.5423319339752);

\path [draw=blue, semithick]
(axis cs:10,-19.3023089170456)
--(axis cs:10,-17.680322766304);

\path [draw=blue, semithick]
(axis cs:20,-24.3779525756836)
--(axis cs:20,-22.7179641723633);

\path [draw=blue, semithick]
(axis cs:30,-25.8785614967346)
--(axis cs:30,-24.6319060325623);
\begin{comment}
\addplot [semithick, goldenrod1911910, line width=1.0, mark=square, mark size=4, mark options={solid,fill opacity=0}]
table {%
0 -11.0885810852051
10 -17.5645446777344
20 -24.433422088623
30 -27.7740230560303
};
\addlegendentry{$\text{UKF}$}
\end{comment}
\addplot [semithick, red, mark=diamond, mark size=5, line width=1.0, mark options={solid,fill opacity=0}]
table {%
0 -11.6274976730347
10 -15.3643646240234
20 -21.1773910522461
30 -23.7296581268311
};
\addlegendentry{$\text{PF}$}
\addplot [semithick, green01270, mark=asterisk, mark size=5,line width=1.0, mark options={solid}]
table {%
0 -4.71466255187988
10 -14.9725952148438
20 -16.4346885681152
30 -15.6540842056274
};
\addlegendentry{$\text{pDANSE}\, (\kappa=0\%)$}
\addplot [semithick, blue, mark=o, mark size=5, line width=1.0, mark options={solid,fill opacity=0}]
table {%
0 -11.1989717483521
10 -18.4913158416748
20 -23.5479583740234
30 -25.2552337646484
};
\addlegendentry{$\text{pDANSE} \, (\kappa=2\%)$}
\end{axis}
\end{tikzpicture}


==> latexmkrc <==
# This shows how to use the xr package with latexmk.
# John Collins 2023-03-29
#
# The xr package ("a system for eXternal References") is used by a document
# to make references to sections, equations, etc in other external
# documents. 
# The definitions in this file enable latexmk to apply latexmk to
# automatically update an external document whenever its .tex file changes,
# so that the references in the main document stay up to date.

# Notes:
#    1. This version is defined to put the files from the compilations of
#       the external documents into a defined subdirectory, to segregate
#       potentially many generated files from the main document
#       directories. 
#    2. But for latexmk's custom dependency mechanism to be used, as here,
#       the aux file from compilation of a subdocument must be generated in
#       the same directory as the corresponding source .tex file.  So the
#       .aux file is copied.
#    3. It is assumed that the external documents are to be compiled by
#       pdflatex.  This can be changed, of course, by changing the '-pdf'
#       option given to the invoked latexmk to whatever is needed.
#    4. An ideal implementation would also ensure that recompilation of an
#       external document also happens whenever any of its other source
#       files changes.  But this is not done in the present version, and
#       would probably entail either the use of internal latexmk variables
#       or extra enhancements to latexmk.
#    5. The code uses subroutines copy and fileparse that are loaded by
#       latexmk from the Perl packages File::Copy and File::Basename.
#    6. It also uses some not-yet-documented features of latexmk: an array
#       variable @file_not_found and subroutines popd, pushd, and
#       rdb_add_generated. 


#--------------------
# Configurable choices for compilation of external documents

# Subdirectory for output files from compilation of external documents:
$sub_doc_output = 'output-subdoc';

# Options to supply to latexmk for compilation of external documents:
@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

#--------------------

# Add a pattern for xr's log-file message about missing files to latexmk's
# list.  Latexmk's variable @file_not_found is not yet documented.
# This line isn't necessary for v. 4.80 or later of latexmk.
push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {
               # In this case, .aux file generated by pdflatex isn't in same
               # directory as the .tex file.
               # Therefore:
               # 1. Actual generated aux file must be listed as produced by this
               #    rule, so that latexmk deals with dependencies correctly.
               #    (Problem to overcome: If $sub_dir_output is same as $aux_dir
               #    for the main document, xr may read the .aux file in the
               #    aux_dir rather than the one the cus dep is assumed by latexmk
               #    to produce, which is in the same directory as the .tex source
               #    file for this custom dependency.)
               #    Use not-yet-documented latexmk subroutine rdb_add_generated
               #    to do this:
               # 2. A copy of the .aux file must be in same directory as .tex file
               #    to satisfy latexmk's definition of a custom dependency.
             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}
